RHINO: Learning Real-Time Humanoid-Human-Object Interaction from Human Demonstrations

Humanoid robots have shown success in locomotion and manipulation. Despite these basic abilities, humanoids are still required to quickly understand human instructions and react based on human interaction signals to become valuable assistants in human daily life. Unfortunately, most existing works only focus on multi-stage interactions, treating each task separately, and neglecting real-time feedback. In this work, we aim to empower humanoid robots with real-time reaction abilities to achieve various tasks, allowing human to interrupt robots at any time, and making robots respond to humans immediately. To support such abilities, we propose a general humanoid-human-object interaction framework, named RHINO, i.e., Real-time Humanoid-human Interaction and Object manipulation. RHINO provides a unified view of reactive motion, instruction-based manipulation, and safety concerns, over multiple human signal modalities, such as languages, images, and motions. RHINO is a hierarchical learning framework, enabling humanoids to learn reaction skills from human-human-object demonstrations and teleoperation data. In particular, it decouples the interaction process into two levels: 1) a high-level planner inferring human intentions from real-time human behaviors; and 2) a low-level controller achieving reactive motion behaviors and object manipulation skills based on the predicted intentions. We evaluate the proposed framework on a real humanoid robot and demonstrate its effectiveness, flexibility, and safety in various scenarios.

==> figs/2_1_classify.tex <==

\begin{figure*}[ht]
    \centering
    % \includegraphics[width=0.8\linewidth]{example-image}
    \includegraphics[width=0.7\linewidth]{figs/src/classify.pdf}
    \caption{\small Illustration to show the importance of interaction data.}
    % \label{fig:intent_corner}
    \label{fig:classify}
\end{figure*}

==> figs/4_1_interaction_corner.tex <==

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.8\linewidth]{example-image}
    \caption{\small Illustration to show the importance of interaction data.}
    \label{fig:intent_corner}
\end{figure}

==> tabs/X_4_skill_hyper.tex <==
\begin{table*}
    \begin{center}
        \caption{Hyper-parameters in real-world deployment across the manipulation tasks. Notes: \textbf{threshold} indicated the \textbf{progress threshold}, \textbf{initial} for \textbf{initial joint position}, \textbf{warm-up} and \textbf{time-out} means the two timings in termination prediction respectively.}
        \label{tab:skill_hyper}
        % \begin{tabular}{c|c|c|c|c|c|c}
        \begin{tabular}{ccccccc}
        \toprule
        \textbf{Scenarios} & \textbf{Object} & \textbf{Task Name} & \begin{tabular}{c}
             \textbf{threshold}  % \\
             % \textbf{threshold}
        \end{tabular} & \begin{tabular}{c}
             \textbf{initial}  % \\
             % \textbf{(Human)}
        \end{tabular} & \begin{tabular}{c}
             \textbf{warm-up}  % \\
             % \textbf{(Human)}
        \end{tabular} & \begin{tabular}{c}
             \textbf{time-out} % \\
             % \textbf{(Human)}
        \end{tabular} \\
            \midrule
            % can
            \multirow{11}{*}{\begin{tabular}{c}
                 Scenario 1 \\
                 Dining Waiter
            \end{tabular}}  & \multirow{2}{*}{can} & Pick Can & $0.85$ & \texttt{predicted} & $2$ & $15$\\
            & & Place Can & $0.85$ & \texttt{fixed} & $2$ & $15$\\
            % plate
            \cmidrule{2-7}
            & \multirow{4}{*}{plate} & Get Plate from Human  & $0.90$ & \texttt{fixed} & $2$ & $15$ \\
            & & Place Plate to Stack & $0.85$ & \texttt{fixed} & $2$ & $15$ \\
            & & Pick Plate from Table & $0.85$ & \texttt{fixed} & $2$ & $15$ \\
            & & Handover Plate & $0.85$ & \texttt{fixed} & $2$ & $15$ \\
            % sponge
            \cmidrule{2-7}
            & \multirow{3}{*}{sponge} & Pick Sponge  & $0.85$ & \texttt{fixed} & $2$ & $15$ \\
            & & Brush with Sponge & \texttt{unused} & \texttt{predicted} & $2$ & $10$ \\
            & & Place Sponge & $0.85$ & \texttt{fixed} & $2$ & $15$ \\
            % tissue
            \cmidrule{2-7}
            & tissue & Pick a Piece of Tissue  & $0.85$ & \texttt{fixed} & $2$ & $15$\\
            \midrule
            % cap
        \multirow{8}{*}{\begin{tabular}{c}
             Scenario 2  \\
             Office Assistant
        \end{tabular}} & \multirow{2}{*}{cap} & Settle Cap & $0.85$ & \texttt{fixed} & $2$ & $15$\\
            & & Handover Cap & $0.85$ & \texttt{predicted} & $2$ & $15$ \\
            % book
            \cmidrule{2-7}
            & book & Pick Book & $0.85$ & \texttt{predicted} & $2$ & $15$ \\
            % stamp
            \cmidrule{2-7}
            & \multirow{3}{*}{stamp} & Pick Stamp & $0.95$ & \texttt{fixed} & $2$ & $15$ \\
            & & Stamp the Paper & $0.85$ & \texttt{predicted} & $2$ & $10$ \\
            & & Place Stamp & $0.85$ & \texttt{predicted} & $2$ & $15$ \\
            % lamp
            \cmidrule{2-7}
            & lamp & Turn off/on the Lamp & $0.85$ & \texttt{fixed} & $2$ & $15$ \\
            % \midrule 
            % \multirow{6}{*}{\begin{tabular}{c}
            %      Expressive Motions
            % \end{tabular}
            % } & \multirow{6}{*}{None} & Cheers & & & $0$ & Dual-Arm\\
            % & & Wave & & & $0$ & Dual-Arm\\
            % & & Shake Hands & & & $0$ & Dual-Arm\\
            % & & Take Photo & & & $0$ & Dual-Arm\\
            % & & Thumb Up & & & $0$ & Dual-Arm\\
            % & & Spread out Hands & & & $0$ & Dual-Arm\\
            \bottomrule
        \end{tabular}
    \end{center}
\end{table*}

==> tabs/X_5_planner.tex <==
\begin{table}
    \begin{center}
     \caption{Hyper-parameters of the Transformer backbone for Reactive Planner.}
        \begin{tabular}{cc}
            \toprule
            hyper-parameter & value \\
            \midrule
            latent dimension  & $128$ \\
            num head &$8$ \\
            num layers & $3$ \\
            batch size & $256$ \\
            feed-forward dimension & $128$ \\
            maximum epoch & $300$ \\
            learning rate & $0.0001$ \\
            \bottomrule
        \end{tabular}
    \end{center}
    \label{tab:planner-hyper}
\end{table}

==> tabs/X_6_motion.tex <==
\begin{table}
    \begin{center}
     \caption{Hyper-parameters of the Interactive Motion Generation Model.}
        \begin{tabular}{cc}
            \toprule
            hyper-parameter & value \\
            \midrule
            latent dimension  & $256$ \\
            num head &$8$ \\
            num layers & $4$ \\
            feed-forward dimension & $256$ \\
            diffusion steps & $300$ \\
            sampling steps & $30$ \\
            batch size & $512$ \\
            maximum epoch & $4000$ \\
            learning rate & $0.0001$ \\
            \bottomrule
        \end{tabular}
    \end{center}
    \label{tab:motion-hyper}
\end{table}
